Partial Mobilization: Tracking Multilingual Information Flows Amongst Russian Media Outlets and Telegram

In response to disinformation and propaganda from Russian online media following the invasion of Ukraine, Russian media outlets such as Russia Today and Sputnik News were banned throughout Europe. To maintain viewership, many of these Russian outlets began to heavily promote their content on messaging services like Telegram. In this work, we study how 16 Russian media outlets interacted with and utilized 732 Telegram channels throughout 2022. Leveraging the foundational model MPNet, DP-means clustering, and Hawkes processes, we trace how narratives spread between news sites and Telegram channels. We show that news outlets not only propagate existing narratives through Telegram but that they source material from the messaging platform. For example, across the websites in our study, between 2.3% (ura.news) and 26.7% (ukraina.ru) of articles discussed content that originated/resulted from activity on Telegram. Finally, tracking the spread of individual topics, we measure the rate at which news outlets and Telegram channels disseminate content within the Russian media ecosystem, finding that websites like ura.news and Telegram channels such as @genshab are the most effective at disseminating their content.

==> conclusion.tex <==
\section{Conclusion}


==> dead.tex <==
\begin{figure}

\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/update_wesbsite_spread.png}
\label{fig:sputnikeban}
\end{subfigure}%

\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/update_wesbsite_spread2.png}
\label{fig:sputnikeban}
\end{subfigure}%
\caption{Spread of narratives/topics amongst Russian websites. As also found in prior work, strategic-Culture.org, in particular, is highly effective at originating ideas/narratives that later appear on other websites~\cite{hanley2022happenstance}.
}
\label{fig:spread-amongst-websites}
\vspace{-10pt}
\end{figure}


%utilizing the intuition that (in the majority of cases) each tweet or telegram messages is about one topic or idea. In contrast, for our set of newspaper articles, we note that each article often contains within it multiple lines of thought, topics, or ideas. For this reason, as in Hanley et al.~\cite{hanley2022happenstance}, we segment each article into its constituent paragraphs.

%The first step of our semantic extraction pipeline leverages a fine-tuned version of MPNet~\cite{song2020mpnet}, which is a 768-dimensional contextual word embedding model released by Microsoft Research. 

%after removing URLs, emojis, and other non-text within the message


%We map each message or tweet to our embedding space,  To do so, we split the articles based on where a newline (\texttt{\escape{n}}) or tab (\texttt{\escape{t}}) character appears within the extracted content. As with our tweets and Telegram messages, we further remove all hyperlinks. Altogether, we embed 2,998,755 distinct Telegram messages from 774 different Telegram channels and 3,375,341 distinct article paragraphs from 18 different websites. 

%To begin, in order to understand the spread of different Russian-state media promoted messages across different platforms, we seek to understand the semantic content within particular articles, messages, and posts. To do so, as in Hanley et al.~\cite{hanley2022happenstance}, we utilize a multilingual version of the large foundational model MPNet~\cite{song2020mpnet}. Embedding each article, message, and tweet utilizing this model, we subsequently examine the similarity of each website, Twitter account, and Telegram channel to each other. 

%After extracting the semantic content of each tweet, article, and telegram message and comparing the content by the community utilizing these mebddings


\begin{figure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/sputnik_telegram_ban.png}
\label{fig:sputnikeban}
\end{subfigure}%
\caption{Example image from Sputniknews.com, directing users to subscribe to Sputnik's international and India telegram channels, as well as providing step-by-step instructions for utilizing a VPN to access their content. 
}
\label{fig:sputnik-ban}
\vspace{-10pt}
\end{figure}



\begin{table*}
\centering
\tiny
\begin{tabular}{l|llllll}
%\toprule

 &\multicolumn{1}{c}{{\textbf{\scriptsize{Telegram}} }} &   &\multicolumn{1}{c}{{\textbf{\scriptsize{Russian Site }}}} &  & \multicolumn{1}{c}{{\textbf{\scriptsize{Shared Telegram} }} } & \# Telegrams\\ 
&  \multicolumn{1}{c}{{\textbf{\scriptsize{Specific Narratives}} }} & \# Telegrams  & \multicolumn{1}{c}{{\textbf{\scriptsize{Specific Narratives}} }}  & \# Articles &  \multicolumn{1}{c}{{\textbf{\scriptsize{and Russian Site Narratives}} }}  & +Articles \\\midrule
  1& The consequences of the shelling  &242 & Hunter Biden had harsh words for former US President Bill Clinton &1571 & Today, Russia attacked the entire territory of Ukraine. & 77,279\\
    & of Dokuchaevsk 24 March  & &and his aides the 2015-2016 email exchange  & & (Russian->English translation) & \\
    & (Russian->English translation) & &  with his long-time business partner Eric Schwerin and Delaware’s,  &\\
    & &  &now-chief deputy attorney general Alexander Mackler, Fox News reports.  &\\
  2 &The answer was not long in coming:   & 239 & The Readovka publication speculated that “The Kyiv Ghost” had to be & 1372 & The UK sanctions will also affect Rostec, UAC, USC,    &  7337\\ 
   &the Kremlin is expelling British diplomats from Russia. &  &sacrificed to refute news that Ukrainian pilots  & & Uralvagonzavod. Sanctions against Belarus will also be introduced.  & \\
   &(Russian->English translation) & & were learning to handle F-16 planes. According to the publication, & &   have been noted  in the Volyn and Poliske directions, \\
     &  && “Western partners” are not very happy with the leak of secret. &&   Britain is ready to provide asylum to the leadership of Ukraine  \\

    & & &  (Spanish -> English Translation) &&  section of the Belarusian-Ukrainian border.\\
  3 & The Ministry of Transport at the congress  & 238 &  Zubets also noted that there was no talk of & 1318 & The demilitarization of Ukraine can take from 5 to 10 years, & 6,152 \\
  &reports today to the president for five years of work & &  western confiscation of Russian assets. It's only about freezing. &&  it is not worth interfering with   \\
 &orally, in writing and on mock-ups.  && Confiscation is an act of war, and  Europe is unlikely && the military and speeding up the special operation. \\
 &(Russian->English translation )  && to ask for serious conflicts with Russia & & (Russian->English translation)\\
\end{tabular}
\caption{\label{tab:shared-disinct-content} The top three narratives--by number of distinct articles or distinct Telegram messages---within the Telegram-specific, the Russian website specific, and the shared Telegram and Russian website ecosystems.  }  
\vspace{-20pt}
\end{table*}


\begin{table}
\centering
\scriptsize
\begin{tabular}{llll}
Top YouTube & \# Telegram  &  Top Twitter &\# Telegram \\ 
 Channels & Channels  &  Accounts  & Channels \\ \midrule
\foreignlanguage{russian}{Россия 24} & 61  & Podolyak\_M & 25\\
\foreignlanguage{russian}{Анатолий Шарий} & 50  &ZelenskyyUa &23\\
Max Chronicler & 46  &elonmusk &23\\
\foreignlanguage{russian}{Комсомольская Правда }  & 39 & DefenceHQ & 22\\
\foreignlanguage{russian}{Информационное агентство БелТА}  & 39 &MelnykAndrij &20\\
\foreignlanguage{russian}{RT на русском}  & 34 &DmytroKuleba & 20 \\
Metametrica  & 34  & vonderleyen &  19\\
Fox News  & 32 &zlj517 & 16\\
\foreignlanguage{russian}{ИЗОЛЕНТА live}   & 31 & defenceu & 15\\
\foreignlanguage{russian}{Телеканал Рада} & 31 & kyivpost & 14\\
SHAMAN & 29& christogrozev  & 13
\end{tabular}
 \caption{\label{tab:top-youtube}Top YouTube and Twitter Accounts Mentioned within our set of 732 Telegram Channels. }  
\vspace{-10pt}
\end{table}

==> ethics-questionaire.tex <==
\subsection{Paper Checklist}

\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
   \answerYes{Yes, our work analyzes news articles in an international context without commenting on any specific culture.}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes. Our abstract is largely reflective of our work.}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes. We outline our  methodology Section~\ref{sec:methoddology} .}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes, in Section~\ref{sec:datasets}, we detail the various aspects of our datasets.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, and we detail the implications and some limitations of our work in the Discussion.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{No, we do not believe that there are any immediate negative social repercussions of our work.}
      \item Did you discuss any potential misuse of your work?
    \answerNo{No; our work is largely an analysis and we see no immediate misuse or negative social repercussions. }
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerNo{No, given the largely analytical nature of our work, we do not see immediate negative social consequences and we have documented the models and methods that we utilize. }
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes.  }
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    \answerNA{NA}
  \item Have you provided justifications for all theoretical results?
    \answerNA{NA}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerNA{NA}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerNA{NA}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerNA{NA}
  \item Have you related your theoretical results to the existing literature in social science?
    \answerNA{NA}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{NA}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Yes, we have included a  GitHub link to the original code for DP-Means clustering from Dinari et al~\cite{dinari2022revisiting}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes, we have outlined these details in Section~\ref{sec:cluster}.}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{We performed clustering so there is not an immediate error bar analysis. However, we did provide an estimated precision of similar content in each cluster. }
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Yes, we have outlined these details in Section~\ref{sec:datasets}.}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerYes{Yes, we have outlined these details in Section~\ref{sec:cluster}.}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
   \answerNA{NA}

  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes, we have included a  GitHub link to the original code for DP-Means clustering from Dinari et al~\cite{dinari2022revisiting}.}
  \item Did you mention the license of the assets?
    \answerNA{NA}
  \item Did you include any new assets in the supplemental material or as a URL?
   \answerNA{NA}

  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
\answerNA{NA}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
   \answerNA{NA}

\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR?
\answerNA{NA}

\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset? 
\answerNA{NA}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerNA{NA}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerNA{NA}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{NA}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerNA{NA}
\end{enumerate}

\end{enumerate}

==> related.tex <==
\vspace{-5pt}
\section{Related Work}

\textit{Circumventing Content Moderation and Censorship:}
Various works have examined users' responses to content moderation and censorship. For instance, in response to the belief that many ``mainstream'' platforms cater to progressive and liberal interests, many ``alternative tech platforms'' like BitChute, MeWe, and Gab have gained popularity~\cite{bhat2022counter}. As found by Miller et~al.\, content moderation often triggers backlashes with users and ``alternative'' platforms often seeking ways to disseminate information ~\cite{miller2022dictatorerdogan}. Han et~al.\, for instance, find that many different websites (\textit{e.g.}, parler.com) are often able to find new hosting services when they are banned from their original ones. Users further often take steps to seek out particular information. Following heavy moderation of QAnon-related subcommunities on the social media website Reddit, many users moved to the Reddit alternative Voat~\cite{hanley2022no}. As shown by Matamoros-Fern{\'a}ndez et~al.\, these alternative platforms with weaker platform and community guidelines are often stores of misinformation and hateful, racist, and violent content~\cite{matamoros2021racism}. Telegram, given its pro-free speech and anti-censorship ideals, for instance, has often attracted content creators and public figures that were banned from other platforms~\cite{rogers2020deplatforming}. In studying these phenomena, H{\"o}hn et~al.\ and Baumgartner et~al.\, for instance, develop public datasets for analyzing the spread of misinformation on Telegram ~\cite{hohn2022belelect,baumgartner2020pushshift}. Similarly, Wich et~al.\ and Hoseini et~al.\ perform case studies of the spread of toxic messages within German and QAnon telegram channels as well~\cite{wich2022introducing,hoseini2021globalization}.


%Despite Telegram being official banned in Russia, for instance, it is often utilized by Russian state media and public officials to influence opinion~\cite{salikov2019telegram}.

%With large social media companies banning violent and harmful content, many have turned towards utilizing decentralized messaging apps to communicate and spread information~\cite{walther2021us}. 

%Both works utilize Google's Perspective API to track the flow of hate, harassment, and otherwise toxic behaviors within these communities. Similarly both utilize large language models and techniques based off Top2Vec~\cite{angelov2020top2vec} and BERTopic~\cite{grootendorst2022bertopic} in order to understand the spread of different ideas within their identified Telegram channels. 

%While Telegram has been the focus of a variety of studies due to its impact, open public channels that broadcast content, its open API, and its 700 million monthly users~\cite{Singh2022}, a substantial amount of work has also investigated the spread of hate and misinformation on WhatsApp. Despite not having open broadcast channels like Telegram, with over 2 billion active monthly users~\cite{Ceci2022}, WhatsApp has inevitably been utilized to share misinformation and hateful content. For instance, Saha et~al.\ find that throughout the 2019 Indian election, WhatsApp was utilized to disseminate Islamophobic content as a rapid clip~\cite{saha2021short}. Similarly, WhatsApp was allegedly utilized as a tool for political radicalization during the Brazilian 2018 election~\cite{evangelista2019whatsapp} and to spread COVID-19 misinformation in Brazil~\cite{soares2021research}.

 







